Communication-Efficient Algorithms For Distributed Optimization

This thesis is concerned with the design of distributed algorithms for solving optimization problems. We consider networks where each node has exclusive access to a cost function, and design algorithms that make all nodes cooperate to find the minimum of the sum of all the cost functions. Several problems in signal processing, control, and machine learning can be posed as such optimization problems. Given that communication is often the most energy-consuming operation in networks, it is important to design communication-efficient algorithms. The main contributions of this thesis are a classification scheme for distributed optimization and a set of corresponding communication-efficient algorithms. The class of optimization problems we consider is quite general, since each function may depend on arbitrary components of the optimization variable, and not necessarily on all of them. In doing so, we go beyond the common assumption in distributed optimization and create additional structure that can be used to reduce the number of communications. This structure is captured by our classification scheme, which identifies easier instances of the problem, for example the standard distributed optimization problem, where all functions depend on all the components of the variable. In our algorithms, no central node coordinates the network, all the communications occur between neighboring nodes, and the data associated with each node is processed locally. We show several applications including average consensus, support vector machines, network flows, and several distributed scenarios for compressed sensing. We also propose a new framework for distributed model predictive control. Through extensive numerical experiments, we show that our algorithms outperform prior distributed algorithms in terms of communication-efficiency, even some that were specifically designed for a particular application.

==> 01-FrontMatter/committee.tex <==


% \newcommand{\spaceadvisors}{\vspace{4.2em}}     % Space between lines
% \newcommand{\spaceadvisorssame}{\vspace{-0.2em}}     % Space between lines
%
%
% \begin{flushleft}
%
%     % ===================================================================================================
%     % Thesis Committee
%     \vspace*{2.0em}
%
%     {\huge \textbf{\sffamily Thesis Committee}}
%
%     \vspace{9.0em}
% 		% ===================================================================================================
%
%
%
% 		% ===================================================================================================
%
% 		% **********************************************
% 		\makebox[16cm][r]{\hrulefill}
%
% 		\makebox[16cm][r]{Pedro Aguiar}
%
% 		\spaceadvisorssame
%
% 		\makebox[16cm][r]{Instituto Superior T\'ecnico}
%
% 		\spaceadvisorssame
%
% 		\makebox[16cm][r]{(Advisor)}
% 		% **********************************************
%
% 		\vfill
%
% 		% **********************************************
% 		\makebox[16cm][r]{\hrulefill}
%
% 		\makebox[16cm][r]{Jos\'e Moura}
%
% 		\spaceadvisorssame
%
% 		\makebox[16cm][r]{Carnegie Mellon University}
% 		% **********************************************
%
% 		\vfill
%
% 		% **********************************************
% 		\makebox[16cm][r]{\hrulefill}
%
% 		\makebox[16cm][r]{Markus P\"uschel}
%
% 		\spaceadvisorssame
%
% 		\makebox[16cm][r]{ETH Zurich \& Carnegie Mellon University}
%
% 		\spaceadvisorssame
%
% 		\makebox[16cm][r]{(Advisor)}
% 		% **********************************************
%
% 		\vfill
%
% 		% **********************************************
% 		\makebox[16cm][r]{\hrulefill}
%
% 		\makebox[16cm][r]{Alejandro Ribeiro}
%
% 		\spaceadvisorssame
%
% 		\makebox[16cm][r]{University of Pennsylvania}
% 		% **********************************************
%
% 		\vfill
%
% 		% **********************************************
% 		\makebox[16cm][r]{\hrulefill}
%
% 		\makebox[16cm][r]{Jo\~ao Xavier}
%
% 		\spaceadvisorssame
%
% 		\makebox[16cm][r]{Instituto Superior T\'ecnico}
%
% 		\spaceadvisorssame
%
% 		\makebox[16cm][r]{(Advisor)}
% 		% **********************************************
%
%     % ===================================================================================================
%
% \end{flushleft}

\newcommand{\spaceadvisors}{\vspace{0.1em}}

\vspace*{0.5cm}

\begin{flushleft}
	\textit{\large Doctoral Dissertation Committee:} \vspace{0.17em}\\

	Professor \textsc{Pedro Aguiar} (Advisor), Instituto Superior T\'ecnico, Technical University of Lisbon  \spaceadvisors \\

	Professor \textsc{Jos\'e M.\ F.\ Moura}, Carnegie Mellon University \spaceadvisors \\

	Professor \textsc{Markus P\"uschel} (Advisor), ETH Zurich \& Carnegie Mellon University \spaceadvisors \\

	Professor \textsc{Alejandro Ribeiro}, University of Pennsylvania \spaceadvisors \\

	Professor \textsc{Jo\~ao Xavier} (Advisor), Instituto Superior T\'ecnico, Technical University of Lisbon


\end{flushleft}


\restoregeometry

\cleardoublepage

==> 01-FrontMatter/cover.tex <==
% =======================================================================================================
% Cover of the thesis:
%   Title
%   Presented by
%   Accepted by the departments of
%   Approved by the college council
% =======================================================================================================

% Formatting
\pagestyle{empty}
\newgeometry{top=1.0in,
bottom=1.0in,
left=1.0in,
right=1.0in}

\newcommand{\spacebetweenlines}{\vspace{1.9em}}     % Space between lines

\begin{center}

    % ===================================================================================================
    % Carnegie Mellon University: CIT
    \vspace{-3.5em}
    {\huge \textbf{\sffamily Carnegie Mellon University}}

    \vspace{1.60em}

    {\large \sffamily CARNEGIE INSTITUTE OF TECHNOLOGY}
    % ===================================================================================================

    % ===================================================================================================
    % Thesis submitted ... Doctor of Philosophy
    \vspace{2.4em}

    {\sffamily THESIS}

    \vspace{1.0em}
    {\sffamily SUBMITTED IN PARTIAL FULFILLMENT OF THE REQUIREMENTS}

    \vspace{1.00em}
    {\sffamily FOR THE DEGREE OF {\large \textbf{DOCTOR OF PHILOSOPHY}}}
    % ===================================================================================================

    % ===================================================================================================
    % Title
    \vspace{3.2em}

    \begin{flushleft}
			\makebox[3.00cm][l]{\textbf{\sffamily \small TITLE}} \hrulefill

			\spacebetweenlines

			\makebox[3.00cm][l]{ } \hrulefill
		\end{flushleft}
    % ===================================================================================================

    % ===================================================================================================
    % Presented by
    \vfill

    \begin{flushleft}
			\makebox[3.00cm][l]{\textbf{\sffamily \small PRESENTED BY}} \hrulefill
    \end{flushleft}

    % ===================================================================================================

    % ===================================================================================================
    % Accepted by the departments of
    \vfill

    \begin{flushleft}
			{\textbf{\sffamily \small ACCEPTED BY THE DEPARTMENTS OF}}

			\spacebetweenlines

			\makebox[3.00cm][l]{ } \hrulefill

			\spacebetweenlines

			\makebox[3.00cm][l]{ } \hrulefill

      % ===============================================================
			% Advisor, Major Professor, Department head 1, Department head 2
			% ===============================================================

			\spacebetweenlines

			% Advisor
			\makebox[3.00cm][l]{ } \makebox[9.1cm]{\hrulefill} \hspace{0.6cm} \hrulefill

			\vspace{-0.22cm}

			\makebox[12.2cm][r]{\footnotesize \sffamily ADVISOR, MAJOR PROFESSOR} \makebox[4.16cm][r]{\footnotesize \sffamily DATE}

			% Department head 1
			\spacebetweenlines

			\makebox[3.00cm][l]{ } \makebox[9.1cm]{\hrulefill} \hspace{0.6cm} \hrulefill

			\vspace{-0.22cm}

			\makebox[12.2cm][r]{\footnotesize \sffamily DEPARTMENT HEAD} \makebox[4.16cm][r]{\footnotesize \sffamily DATE}

			% Department head 2
			\spacebetweenlines

			\makebox[3.00cm][l]{ } \makebox[9.1cm]{\hrulefill} \hspace{0.6cm} \hrulefill

			\vspace{-0.22cm}

			\makebox[12.2cm][r]{\footnotesize \sffamily DEPARTMENT HEAD} \makebox[4.16cm][r]{\footnotesize \sffamily DATE}
    \end{flushleft}
    % ===================================================================================================

    % ===================================================================================================
    % Approved by the college council
    \vfill

		\begin{flushleft}
			{\textbf{\sffamily \small APPROVED BY THE COLLEGE COUNCIL}}

			\spacebetweenlines

			\makebox[3.00cm][l]{ } \makebox[9.1cm]{\hrulefill} \hspace{0.6cm} \hrulefill

			\vspace{-0.22cm}

			\makebox[12.2cm][r]{\footnotesize \sffamily DEAN} \makebox[4.16cm][r]{\footnotesize \sffamily DATE}
		\end{flushleft}
    % ===================================================================================================
\end{center}


\cleardoublepage


==> 01-FrontMatter/titlepage.tex <==

\newgeometry{top=1.0in,
bottom=1.0in,
left=1.0in,
right=1.0in}

\newcommand{\spacebetweenlinesT}{\vspace{0.1em}}     % Space between lines

\begin{titlepage}
    \begin{flushleft}

    \vspace*{0.2cm}

    {\Huge \textbf{Communication-Efficient Algorithms \vspace{0.4em}\\For Distributed Optimization}}

    \vspace{4.0em}

    {\large \textsc{Jo\~ao F. C. Mota}} \vspace{0.5em}

    {\large \today}

    \vfill

		\psscalebox{1.05}{
		\begin{pspicture}(8,5.0)
				\def\nodesimp{
            \pscircle*[linecolor=black!50!white](0,0){0.3}
        }
        \rput(1,3.7){\rnode{N1}{\nodesimp}}
        \rput(0.3,2){\rnode{N2}{\nodesimp}}
        \rput(0.3,0.3){\rnode{N3}{\nodesimp}}
        \rput(2.5,1.7){\rnode{N4}{\nodesimp}}
        \rput(5,2){\rnode{N5}{\nodesimp}}
        \rput(3.8,3){\rnode{N6}{\nodesimp}}
        \rput(6.7,3.2){\rnode{N7}{\nodesimp}}
        \rput(3.5,0.5){\rnode{N8}{\nodesimp}}
        \rput(6.3,0.9){\rnode{N9}{\nodesimp}}
        \rput(4.1,4.1){\rnode{N10}{\nodesimp}}

        \ncline[nodesep=0.37cm]{-}{N1}{N2}
        \ncline[nodesep=0.37cm]{-}{N1}{N4}
        \ncline[nodesep=0.37cm]{-}{N2}{N3}
        \ncline[nodesep=0.37cm]{-}{N2}{N4}
        \ncline[nodesep=0.37cm]{-}{N4}{N5}
        \ncline[nodesep=0.37cm]{-}{N4}{N6}
        \ncline[nodesep=0.37cm]{-}{N5}{N6}
        \ncline[nodesep=0.37cm]{-}{N5}{N7}
        \ncline[nodesep=0.37cm]{-}{N3}{N4}
        \ncline[nodesep=0.37cm]{-}{N1}{N6}
        \ncline[nodesep=0.37cm]{-}{N6}{N7}
        \ncline[nodesep=0.37cm]{-}{N8}{N4}
        \ncline[nodesep=0.37cm]{-}{N8}{N5}
        \ncline[nodesep=0.37cm]{-}{N8}{N9}
        \ncline[nodesep=0.37cm]{-}{N8}{N3}
        \ncline[nodesep=0.37cm]{-}{N8}{N6}
        \ncline[nodesep=0.37cm]{-}{N9}{N5}
        \ncline[nodesep=0.37cm]{-}{N9}{N7}
        \ncline[nodesep=0.37cm]{-}{N10}{N6}
        \ncline[nodesep=0.37cm]{-}{N10}{N7}
        \ncline[nodesep=0.37cm]{-}{N10}{N1}
        \ncline[nodesep=0.37cm]{-}{N10}{N5}

        %\psgrid
		\end{pspicture}
		}

		\vfill

    {\large
		\emph{A Dissertation Submitted in Partial Fulfillment of the}  \spacebetweenlinesT\\
		\emph{Requirements for the Degree of Doctor of Philosophy 	in}
    }

    \vspace{0.4em}

    {\large
			Electrical and Computer Engineering 	\spacebetweenlinesT \\
			Carnegie Mellon University, 	Pittsburgh, PA \spacebetweenlinesT \\
			Instituto Superior T\'ecnico, Technical University of Lisbon, Portugal
		}

		\vfill

		{\large
			\textit{Co-advised by:}	\spacebetweenlinesT \\
			Pedro Aguiar, Instituto Superior T\'ecnico, Technical University of Lisbon \spacebetweenlinesT \\
			Markus P\"uschel, ETH Zurich \& Carnegie Mellon University \spacebetweenlinesT \\
			Jo\~ao Xavier, Instituto Superior T\'ecnico, Technical University of Lisbon
		}

    \end{flushleft}
    %\vspace{1.0cm}

\end{titlepage}

\restoregeometry

==> 01-FrontMatter/titlepageCMU.tex <==

\newgeometry{top=1.0in,
bottom=1.0in,
left=1.0in,
right=1.0in}

\newcommand{\spacebetweenlinesT}{\vspace{0.1em}}     % Space between lines

\begin{titlepage}
    \begin{center}

    \vspace*{1cm}

    {\huge \textbf{Communication-Efficient Algorithms \vspace{0.4em}\\For Distributed Optimization}}

    \vfill

    {\large
		Submitted in partial fulfillment of the requirements  for \spacebetweenlinesT\\
		for the degree of  \vspace{0.5em} \\
		{\Large Doctor of Philosophy}  \spacebetweenlinesT \\
		{\Large in} \spacebetweenlinesT \\
		{\Large Electrical and Computer Engineering}
    }

    \vfill

    {\large \textsc{Jo\~ao F. C. Mota}}

    \vspace{0.7cm}

    {\large M.\ S., Electrical and Computer Engineering, Instituto Superior T\'ecnico, Portugal}
    \spacebetweenlinesT \\
    {\large B.\ S., Electrical and Computer Engineering, Instituto Superior T\'ecnico, Portugal}


		\vfill

		{\large Carnegie Mellon University \spacebetweenlinesT \\ Pittsburgh, PA}

		\vspace{0.7cm}

		{\large \today}


    \end{center}
    %\vspace{1.0cm}

\end{titlepage}

\restoregeometry

==> 02-MainMatter/classification.tex <==

\chapter{A Classification Scheme For Distributed Optimization}
\label{Ch:Classification}

	This chapter introduces a classification scheme for optimization problems formulated on networks. The scheme will help us organize and categorize the vast prior work on distributed optimization, in Chapter~\ref{Ch:relatedWork}. Additionally, it will serve as a building block for our algorithms. Before we define the classes of problems, we need to introduce two fundamental concepts. First, we need the concept of \textit{communication network}, which will represent the physical network through which the nodes exchange messages. Second, we need to establish the relationship between each node and the variable of the optimization problem. This will be done using what we call \textit{variable classification}. While variable classification alone will define the class of a problem, the structure of the communication network will determine special cases within each class. This is be done in Section~\ref{Sec:FundamentalConcepts}. Then, in Section~\ref{Sec:ClassesOptimProblems}, we analyze each problem class and show the relevance of the proposed classification scheme to achieve the goals of this thesis. Finally, in Section~\ref{Sec:ConnectedAndNonConnectedSubclasses} we discuss the special cases within each class, i.e., the classification subclasses.


\section{Fundamental concepts}
\label{Sec:FundamentalConcepts}

	\subsection{Communication network}
	\label{SubSec:CommunicationNetwork}

	The communication network is the physical network through which the computing devices, seen as network nodes, communicate. We represent the communication network with an undirected graph~$\mathcal{G}=(\mathcal{V},\mathcal{E})$, where $\mathcal{V}$ and $\mathcal{E}$ are the set of nodes and the set of edges, respectively. The cardinality of these sets, i.e., the number of nodes and the number of edges, will be denoted with~$P=|\mathcal{V}|$ and~$E=|\mathcal{E}|$, respectively. \fref{Fig:IntroNetwork} in \cref{Ch:Introduction} shows an example of a graph representing a communication network with~$P=10$ nodes and~$E = 21$ edges. An edge belongs to the communication network, say $(i,j) \in \mathcal{E}$, if and only if nodes~$i$ and~$j$ communicate directly. For example, nodes~$1$ and~$10$ in \fref{Fig:IntroNetwork} are neighbors: this means they can exchange messages with each other, because there is a communication link connecting them. We use the following convention: if~$(i,j) \in \mathcal{E}$, then~$i<j$.

	\mypar{Functions associated to nodes}
  Associated with each node, there is a function depending on the components of a variable~$x \in \mathbb{R}^n$. The function at node~$p$ is denoted with $f_p:\mathcal{D}_p \subseteq \mathbb{R}^{n} \xrightarrow{} \mathbb{R} \cup \{+\infty\}$ and, unless otherwise stated, we assume it is closed and convex~\cite{Boyd04-ConvexOptimization,BenTal01-LecturesModernConvexOptimization,Bertsekas99-NonlinearProgramming,Lemarechal04-FundamentalsConvexAnalysis,Nesterov04-IntroductoryLecturesConvexOptimization}. Note that each function~$f_p$ can take the value~$+\infty$ and, therefore, node~$p$ can impose constraints on the variable~$x$ implicitly, via indicator functions. An indicator function of a given set~$S \subset \mathbb{R}^n$ is defined as $\text{i}_S:\mathbb{R}^n \xrightarrow{} \mathbb{R} \cup \{+\infty\}$,
  $$
		\text{i}_S(x) =
		\left\{
			\begin{array}{ll}
				0 &,\,\, x \in S \\
				+\infty &,\,\, x \not\in S\,.
			\end{array}
		\right.
  $$
  Including an indicator function $\text{i}_S(x)$ in the objective of a minimization problem forces $x \in S$, since otherwise the optimal (minimal) value is~$+\infty$. Each function~$f_p$ is \textit{private}, i.e., at all times during and before the execution of the algorithm, only node~$p$ knows~$f_p$. As explained before, this privacy rule formalizes our wish to derive a distributed algorithm by enforcing local computations; namely, all computations involving~$f_p$ have to be done at node~$p$. This makes sense in scenarios where each~$f_p$ encodes a database that should be known only at node~$p$, or simply to make use of all the distributed computing resources as, for example, in a sensor network, where each sensor has some processing power available for computation.

  \subsection{Variable classification}

	Although each function is uniquely associated to a single node, the same does not happen for each component of~$x \in \mathbb{R}^n$, the problem variable. This originates several scenarios and motivates the classification scheme we devise in this chapter. Part of our strategy is to classify each component of the variable~$x$ according to the properties of its induced subgraph.

  \begin{figure}[h]
  \centering
  \subfigure[Partial connected variable]{\label{SubFig:ClassLocalVariable}
    \psscalebox{0.9}{
      \begin{pspicture}(4.9,4.8)
        \def\nodesimp{
          \pscircle*[linecolor=black!65!white](0,0){0.3}
        }

        \rput(0.5,4.1){\rnode{C1}{\nodesimp}}   \rput(0.5,4.1){\small \textcolor{white}{$1$}}
        \rput(1.0,2.6){\rnode{C2}{\nodesimp}}   \rput(1.0,2.6){\small \textcolor{white}{$2$}}
        \rput(0.9,0.9){\rnode{C3}{\nodesimp}}   \rput(0.9,0.9){\small \textcolor{white}{$3$}}
        \rput(3.1,1.1){\rnode{C4}{\nodesimp}}   \rput(3.1,1.1){\small \textcolor{white}{$4$}}
        \rput(4.1,2.6){\rnode{C5}{\nodesimp}}   \rput(4.1,2.6){\small \textcolor{white}{$5$}}
        \rput(2.3,3.3){\rnode{C6}{\nodesimp}}   \rput(2.3,3.3){\small \textcolor{white}{$6$}}

        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C2}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C3}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C3}{C4}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C4}{C5}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C5}{C6}

        \rput[lb](-0.1,4.45){\small $f_1(x_1,x_2)$}
        \rput[lt](1.2,2.4){\small $f_2(x_1,x_2,x_3)$}
        \rput[lt](0,0.56){\small $f_3(x_2,x_3)$}
        \rput[t](3.1,0.74){\small $f_4(x_3)$}
        \rput[b](4.2,2.97){\small $f_5(x_1,x_3)$}
        \rput[b](2.7,3.65){\small $f_6(x_1,x_2)$}

        %\psgrid
      \end{pspicture}
    }
  }
  \hfill
  \subfigure[Subgraph induced by $x_2$]{\label{SubFig:ClassLocalVariableHighlighted}
    \psscalebox{0.9}{
      \begin{pspicture}(4.9,4.8)
        \def\nodesimp{
          \pscircle*[linecolor=black!65!white](0,0){0.3}
        }
        \def\nodeshigh{
          \pscircle*[linecolor=black!25!white](0,0){0.3}
        }

        \rput(0.5,4.1){\rnode{C1}{\nodesimp}}    \rput(0.5,4.1){\small \textcolor{white}{$1$}}
        \rput(1.0,2.6){\rnode{C2}{\nodesimp}}    \rput(1.0,2.6){\small \textcolor{white}{$2$}}
        \rput(0.9,0.9){\rnode{C3}{\nodesimp}}    \rput(0.9,0.9){\small \textcolor{white}{$3$}}
        \rput(3.1,1.1){\rnode{C4}{\nodeshigh}}   \rput(3.1,1.1){\small \textcolor{black!60!white}{$4$}}
        \rput(4.1,2.6){\rnode{C5}{\nodeshigh}}   \rput(4.1,2.6){\small \textcolor{black!60!white}{$5$}}
        \rput(2.3,3.3){\rnode{C6}{\nodesimp}}    \rput(2.3,3.3){\small \textcolor{white}{$6$}}

        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C2}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C3}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C3}{C4}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C4}{C5}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C5}{C6}

        \rput[lb](-0.1,4.45){\small $f_1(x_1,\boldsymbol{x_2})$}
        \rput[lt](1.2,2.4){\small $f_2(x_1,\boldsymbol{x_2},x_3)$}
        \rput[lt](0,0.56){\small $f_3(\boldsymbol{x_2},x_3)$}
        \rput[t](3.1,0.74){\small \textcolor{black!70!white}{$f_4(x_3)$}}
        \rput[b](4.2,2.97){\small \textcolor{black!70!white}{$f_5(x_1,x_3)$}}
        \rput[b](2.7,3.65){\small $f_6(x_1,\boldsymbol{x_2})$}

        %\psgrid
      \end{pspicture}
    }
  }
  \hfill
  \subfigure[Mixed connected variable]{\label{SubFig:ClassMixedVariable}
    \psscalebox{0.9}{
      \begin{pspicture}(4.9,4.8)
        \def\nodesimp{
          \pscircle*[linecolor=black!65!white](0,0){0.3}
        }

        \rput(0.5,4.1){\rnode{C1}{\nodesimp}}   \rput(0.5,4.1){\small \textcolor{white}{$1$}}
        \rput(1.0,2.6){\rnode{C2}{\nodesimp}}   \rput(1.0,2.6){\small \textcolor{white}{$2$}}
        \rput(0.9,0.9){\rnode{C3}{\nodesimp}}   \rput(0.9,0.9){\small \textcolor{white}{$3$}}
        \rput(3.1,1.1){\rnode{C4}{\nodesimp}}   \rput(3.1,1.1){\small \textcolor{white}{$4$}}
        \rput(4.1,2.6){\rnode{C5}{\nodesimp}}   \rput(4.1,2.6){\small \textcolor{white}{$5$}}
        \rput(2.3,3.3){\rnode{C6}{\nodesimp}}   \rput(2.3,3.3){\small \textcolor{white}{$6$}}

        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C2}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C3}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C3}{C4}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C4}{C5}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C5}{C6}

        \rput[lb](-0.1,4.45){\small $f_1(x_1,x_2)$}
        \rput[lt](1.2,2.4){\small $f_2(x_1,x_2,x_3)$}
        \rput[lt](0.2,0.56){\small $f_3(x_1,x_3)$}
        \rput[t](3.1,0.74){\small $f_4(x_1)$}
        \rput[b](4.2,2.97){\small $f_5(x_1,x_2)$}
        \rput[b](2.7,3.65){\small $f_6(x_1,x_2)$}

        %\psgrid
      \end{pspicture}
    }
  }
  \caption{
    Example of \text{(a)} a partial connected variable and \text{(c)} a mixed connected variable. \text{(b)} highlights the subgraph induced by the component~$x_2$ in \text{(a)}. The communication network is the same in all cases. In \text{(c)}, the component~$x_1$ is global, and~$x_2$ and~$x_3$ induce connected subgraphs.
  }
  \label{Fig:ClassificationExamplesVariable}
  \end{figure}


	\mypar{Induced subgraph}
	Let~$x_l \in \mathbb{R}$ denote the $l$th component of the optimization variable~$x \in \mathbb{R}^n$, for $l=1,\ldots,n$.	We define the subgraph induced by~$x_l$ similarly to how~\cite[Ch.1]{Bollobas08-ModernGraphTheory} defines the subgraph induced by a set of nodes. In our case, these nodes are the ones whose functions depend on~$x_l$. To be more concrete, given a communication network~$\mathcal{G}$, the \textit{subgraph induced by $x_l$} is the subgraph $\mathcal{G}_l = (\mathcal{V}_l,\mathcal{E}_l) \subseteq \mathcal{G}$, where $\mathcal{V}_l$ is the set of nodes whose functions depend on~$x_l$, and an edge $(i,j)$ belongs to~$\mathcal{E}_l$ only if $(i,j) \in \mathcal{E}$ and both nodes~$i$ and~$j$ belong to~$\mathcal{V}_l$. As an example, \fref{SubFig:ClassLocalVariableHighlighted} highlights the subgraph induced by the component~$x_2$ in the setting of \fref{SubFig:ClassLocalVariable}: the set of nodes and the set of edges of this induced subgraph~$\mathcal{G}_2$ are, respectively, $\mathcal{V}_2 = \{1,2,3,6\}$ and $\mathcal{E}_2 = \{(1,2),(1,6),(2,3),(2,6)\}$. Note that neither~$f_4$ nor~$f_5$ depend on~$x_2$.

	\mypar{Component classification}
	We define two attributes for a given component~$x_l$, according to the properties of its induced subgraph~$\mathcal{G}_l$. The first attribute uses only information of the function dependencies, i.e., whether all functions depend on~$x_l$ or not. Namely, we say that~$x_l$ is
	\begin{itemize}
		\item \textit{Global} if $\mathcal{G}_l$ coincides with the communication network~$\mathcal{G}$, i.e., $\mathcal{G}_l = \mathcal{G}$;
		\item \textit{Partial} if $\mathcal{G}_l$ is a strict subgraph of~$\mathcal{G}$, i.e., $\mathcal{G}_l \subset \mathcal{G}$.
	\end{itemize}
	In other words, the component~$x_l$ is global if the functions of all nodes depend on~$x_l$, and it is partial if there is at least one function that does not depend on~$x_l$. For example, in \fref{SubFig:ClassMixedVariable}, $x_1$ is a global component because it appears in all nodes, while~$x_2$ is a partial component because neither~$f_3$ nor~$f_4$ depend on it.

	The second attribute uses information about the network topology, namely, the connectivity of $\mathcal{G}_l$. We say that~$x_l$ is
	\begin{itemize}
		\item \textit{Connected} if $\mathcal{G}_l$ is connected, i.e., if there is a path between any pair of nodes in $\mathcal{G}_l$;
		\item \textit{Non-connected} if $\mathcal{G}_l$ is not connected, i.e., if there are at least two nodes in~$\mathcal{G}_l$ for which no connecting path exists.
	\end{itemize}
	For example, the (highlighted) subgraph induced by~$x_2$ in \fref{SubFig:ClassLocalVariableHighlighted} is connected and, thus, $x_2$ is connected. The same can be verified for the components $x_1$ and~$x_3$ in \fref{SubFig:ClassLocalVariable} and for the components $x_2$ and~$x_3$ in \fref{SubFig:ClassMixedVariable}. Naturally, a global component is always connected, since its induced subgraph coincides with the communication network, which we assume connected.

	\begin{figure}[h]
  \centering
  \psscalebox{1.05}{
    \begin{pspicture}(9,3.4)

        \psframe*[linecolor=black!7!white](-0.2,-0.21)(9.2,3.3)
        \psframe*[linecolor=black!20!white](-0.05,1.3)(9.05,2.2)
        \psframe*[linecolor=black!20!white](1.2,0)(9.05,0.9)

        \rput(4,3){\rnode{N1}{\textsf{\footnotesize variable} \small $x$}}
        \rput(1,1.7){\rnode{N2}{\textsf{\footnotesize global}}}
        \rput(3,1.7){\rnode{N3}{\textsf{\footnotesize partial}}}
        \rput(7,1.7){\rnode{N4}{\textsf{\footnotesize mixed}}}

        \rput(2,0.4){\rnode{N5}{\textsf{\footnotesize connected}}}
        \rput(4,0.4){\rnode{N6}{\textsf{\footnotesize non-connected}}}
        \rput(6,0.4){\rnode{N7}{\textsf{\footnotesize connected}}}
        \rput(8,0.4){\rnode{N8}{\textsf{\footnotesize non-connected}}}

        \ncline[nodesep=0.08cm]{-}{N1}{N2}
        \ncline[nodesep=0.08cm]{-}{N1}{N3}
        \ncline[nodesep=0.08cm]{-}{N1}{N4}
        \ncline[nodesep=0.08cm]{-}{N3}{N5}
        \ncline[nodesep=0.08cm]{-}{N3}{N6}
        \ncline[nodesep=0.08cm]{-}{N4}{N7}
        \ncline[nodesep=0.08cm]{-}{N4}{N8}

        \rput[rt](8.95,2.13){\scriptsize \textit{\textsf{\textcolor{white}{\textbf{Level 1}}}}}
        \rput[rt](8.95,0.83){\scriptsize \textit{\textsf{\textcolor{white}{\textbf{Level 2}}}}}
        %\psgrid
   \end{pspicture}
  }
  \medskip
  \caption{Classification of the variable~$x$. In level~$1$, $x$ is classified according to the relation between each component and the function at each node. Level~$2$ uses information about the network structure to classify~$x$ with further granularity.}
  \label{Fig:Classification}
  \end{figure}

  \mypar{Variable classification}
	With the component-wise classification of components, we are now in conditions to classify the full optimization variable~$x \in \mathbb{R}^n$. The proposed classification scheme is shown in \fref{Fig:Classification} and has two classification levels. In level~$1$, three classes are defined: namely, we say that the variable $x \in \mathbb{R}^n$ is
	\begin{itemize}
		\item \textit{Global} if all its components are global;
		\item \textit{Partial} if all its components are partial;
		\item \textit{Mixed} if it is neither global nor partial, i.e., there is at least one global component and one partial component.
	\end{itemize}
	A mixed variable can always be decomposed into its global and partial parts. Figures~\ref{SubFig:ClassLocalVariable} and~\ref{SubFig:ClassMixedVariable} show examples of a partial and a mixed variable, respectively. The mixed variable in \fref{SubFig:ClassMixedVariable} has a global part~$x_1$ and a partial part~$(x_2,x_3)$. Note that this level~$1$ classification uses information only about the components each function depends on.

	The partial and the mixed classes are further subdivided into two subclasses, connected and non-connected, as shown in \fref{Fig:Classification}. This subdivision arises naturally if we classify the full variable according to the second component-level attribute: we say that $x \in \mathbb{R}^n$ is
	\begin{itemize}
		\item \textit{Connected} if all its components are connected;
		\item \textit{Non-connected} if at least one of its components is non-connected.
	\end{itemize}
	As said before, a global variable is always connected because all its components appear in every function, and the communication network is assumed connected. This is the reason why level~$2$ classification does not apply to a global variable (cf.\ \fref{Fig:Classification}). A mixed variable, though, will only be connected if all the components of its partial part are connected. For example, the mixed variable of \fref{SubFig:ClassMixedVariable} is connected because $x_1$ is a global component and~$x_2$ and~$x_3$ are partial components that induce connected graphs.


\section{Classes of optimization problems}
\label{Sec:ClassesOptimProblems}

	Knowing how to classify a variable, we are now in conditions to define our classes of distributed optimization problems. In all these problems, the goal is to minimize the sum of all the functions. We thus define a problem class according to the class of the respective optimization variable:
  \begin{align}
		  \label{Eq:GlobalProblem}\tag{G}
			\text{\textit{Global Problem:}}
		&\qquad\qquad\qquad
			\begin{array}{ll}
				\underset{x \in \mathbb{R}^n}{\text{minimize}} & f_1(x) + f_2(x) + \cdots + f_P(x)
			\end{array}
			\qquad\qquad
   \\
			\label{Eq:PartialProblem}\tag{P}
			\text{\textit{Partial Problem:}}
    &\qquad\qquad\qquad
			\begin{array}{ll}
				\underset{x \in \mathbb{R}^n}{\text{minimize}} & f_1(x_{S_1}) + f_2(x_{S_2}) + \cdots + f_P(x_{S_P})
			\end{array}
			\hfill
    \\
			\label{Eq:MixedProblem}\tag{M}
			\text{\textit{Mixed Problem:}}
    &\qquad\qquad\qquad
			\begin{array}{ll}
				\underset{x = (y,z) \in \mathbb{R}^n}{\text{minimize}} & f_1(y, z_{S_1}) + f_2(y, z_{S_2}) + \cdots + f_P(y, z_{S_P})
			\end{array}
			\qquad
  \end{align}
  The optimization variable~$x$ is global in~\eqref{Eq:GlobalProblem}, partial in~\eqref{Eq:PartialProblem}, and mixed in~\eqref{Eq:MixedProblem}. We thus see how level~$1$ classification in \fref{Fig:Classification} yielded our three classes of problems. In~\eqref{Eq:PartialProblem} and in~\eqref{Eq:MixedProblem} we used the following notation: for any vector~$v \in \mathbb{R}^n$ and any subset~$S \subseteq \{1,2,\ldots,n\}$, $v_S$ represents the components of~$v$ indexed by the set~$S$. For example, if~$v \in \mathbb{R}^5$ and~$S = \{2,4,5\}$, then~$v_S = (v_2,v_4,v_5)$. Hence, the set~$S_p$  encodes the dependency of function~$f_p$ on the components of~$x$. By using this notation, we assume $S_1 \cap S_2 \cap \cdots \cap S_P = \emptyset$, otherwise~\eqref{Eq:PartialProblem} could have global components and the classes would not be clearly distinct. We also assume that $S_1 \cup S_2 \cup \cdots \cup S_P = \{1,\ldots,n\}$, i.e., that each component~$x_l$ appears in at least one of the sets~$S_p$. Note that this does not imply that the sets $S_1$, $S_2$,\ldots, $S_P$ form a partition of $\{1,\ldots,n\}$: that would only hold if the pairwise intersections $S_i \cap S_j$ were empty which, in general, are not. The mixed variable in~\eqref{Eq:MixedProblem} was explicitly partitioned into its global part~$y$ and into its partial part~$z$. The challenge in solving any of the above classes is that each node in the network knows only one term of the objective (its private function) and can only communicate with its neighbors. Yet, all nodes have to cooperate in order to agree on a solution for the problem at hand. Such solution will be denoted with~$x^\star$ for either~\eqref{Eq:GlobalProblem}, \eqref{Eq:PartialProblem}, or~\eqref{Eq:MixedProblem}.

  \mypar{Encoding constraints}
  At first sight, the classes~\eqref{Eq:GlobalProblem}, \eqref{Eq:PartialProblem}, and \eqref{Eq:MixedProblem} defined above seem to be limited to problems with no constraints. Recall, however, that each function can take the value~$+\infty$, since $f_p: \mathcal{D}_p \subseteq \mathbb{R}^n \xrightarrow{} \mathbb{R} \cup \{+\infty\}$. Therefore, we can use indicator functions to encode constraints in the optimization problems. Suppose, for example, that node~$p$ has a function $\overline{f}_p(x_{S_p^1})$ and wants to constrain the set of components $x_{S_p^2}$ as $h_p(x_{S_p^2}) = 0$, where $S_p^1$ and~$S_p^2$ are arbitrary subsets of~$\{1,\ldots,n\}$. Then, just define the function of node~$p$ as $f_p(x_{S_p}) = \overline{f}_p(x_{S_p^1}) + \text{i}_{h_p}(x_{S_p^2})$, where $S_p = S_p^1 \cup S_p^2$ and $\text{i}_{h_p=0}(x_{S_p^2})$ is a shorthand for the indicator function of the set $\{x_{S_p^2}\,:\, h_p(x_{S_p^2}) = 0\}$. An obvious consequence is that we can encode arbitrary constraints in the optimization problems~\eqref{Eq:GlobalProblem}, \eqref{Eq:PartialProblem}, and \eqref{Eq:MixedProblem}. Another less obvious consequence is that by allowing $+\infty$ values, we also make all these problem classes equivalent. We show next, however, that, in spite of this equivalence, in distributed scenarios each class has to be addressed separately for communication-efficiency reasons.


  \subsection{Relevance of our classification scheme}

  In this subsection we show that the proposed classification scheme is relevant for the design of distributed algorithms. First, we show that all the classes, \eqref{Eq:GlobalProblem}, \eqref{Eq:PartialProblem}, and~\eqref{Eq:MixedProblem} actually represent the same set of problems. Although this might indicate that the classification scheme is useless, we then show it is not. The reason is that reformulating a problem in a given class into a problem in another class, for example, a problem in~\eqref{Eq:GlobalProblem} into a problem in~\eqref{Eq:PartialProblem}, will invariably introduce unnecessary communications in the distributed algorithm. Therefore, if communication-efficiency is a design specification, one has to address the problem classes separately.

  \mypar{Equivalence between problem classes}
  Using the concept of \textit{problem equivalence} as defined in~\cite[\S4.1.3]{Boyd04-ConvexOptimization}, we now show that problems~\eqref{Eq:GlobalProblem}, \eqref{Eq:PartialProblem}, and~\eqref{Eq:MixedProblem} are equivalent:

  \begin{lemma}[Equivalence between problem classes]
  \label{lem:EquivalenceBetweenClasses}
  \hfill

  \medskip
  \noindent
		Assume problems~\eqref{Eq:GlobalProblem}, \eqref{Eq:PartialProblem}, and~\eqref{Eq:MixedProblem} are defined on a communication network that is connected. Also, assume that the function at each node can take the value $+\infty$ to encode constraints implicitly. Let the variable~$x \in \mathbb{R}^n$ have dimensions $n \geq 2$. Then,
		\newcounter{ClassLemmaEquiv}
		\begin{list}{(\alph{ClassLemmaEquiv})}{\usecounter{ClassLemmaEquiv}}
			\item \eqref{Eq:GlobalProblem} can be written as either \eqref{Eq:PartialProblem} or~\eqref{Eq:MixedProblem}
			\item \eqref{Eq:PartialProblem} can be written as either \eqref{Eq:GlobalProblem} or \eqref{Eq:MixedProblem}
			\item \eqref{Eq:MixedProblem} can be written as either \eqref{Eq:GlobalProblem} or~\eqref{Eq:PartialProblem}.
		\end{list}
  \end{lemma}
  \begin{proof}
  \hfill

  \medskip
  \noindent
		\newcounter{ClassLemmaEquivProof}
		\begin{list}{(\alph{ClassLemmaEquivProof})}{\usecounter{ClassLemmaEquivProof}}
			\item
				There are several way of writing~\eqref{Eq:GlobalProblem} as~\eqref{Eq:PartialProblem}. For example, one can create~$P$ copies of the variable~$x$, i.e., $x_1$, $x_2$, \ldots, $x_P$, and associate the copy~$x_p$ with node~$p$. Denoting the set of neighbors of a node~$p$ by~$\mathcal{N}_p$, \eqref{Eq:GlobalProblem} is written equivalently as
				\begin{equation}\label{Eq:Cl:LemmaProof1}
					\begin{array}{cl}
						\underset{\bar{x} = (x_1,\ldots,x_P)}{\text{minimize}} & f_1(x_1) + f_2(x_2) + \cdots + f_P(x_P) \\
						\text{subject to} & x_p = x_j\,,\quad j \in \mathcal{N}_p\,,\quad p=1,\ldots,P\,.
					\end{array}
				\end{equation}
				The constraints in~\eqref{Eq:Cl:LemmaProof1} enforce all copies to be equal and thus problems~\eqref{Eq:Cl:LemmaProof1} and~\eqref{Eq:GlobalProblem} to be equivalent. The variable in~\eqref{Eq:Cl:LemmaProof1} is the set of the copies $\overline{x} = (x_1,\ldots,x_P) \in (\mathbb{R}^n)^P$. Now, write~\eqref{Eq:Cl:LemmaProof1} equivalently as
				\begin{equation}\label{Eq:Cl:LemmaProof2}
					\begin{array}{ll}
						\underset{\bar{x} = (x_1,\ldots,x_P)}{\text{minimize}} & \bar{f}_1(x_1, \{x_j\}_{j \in \mathcal{N}_1}) + \bar{f}_2(x_2, \{x_j\}_{j \in \mathcal{N}_2}) + \cdots + \bar{f}_P(x_P, \{x_j\}_{j \in \mathcal{N}_P})\,,
					\end{array}
				\end{equation}
				where, for each~$p$, $\bar{f}_p$ is defined as
				\begin{equation}\label{Eq:Cl:LemmaProof3}
					\bar{f}_p(x_p,\{x_j\}_{j \in \mathcal{N}_p}) = f_p(x_p) + \sum_{j \in \mathcal{N}_p} \text{i}_{\{0\}}(x_p - x_j)\,,
				\end{equation}
				and~$\text{i}_{\{0\}}(\cdot)$ is the indicator function of the singleton~$0 \in \mathbb{R}^n$. Problem~\eqref{Eq:Cl:LemmaProof2} clearly has the format of~\eqref{Eq:PartialProblem}.

				To write~\eqref{Eq:GlobalProblem} as~\eqref{Eq:MixedProblem}, use the assumption that $n\geq 2$ and repeat the procedure just described, but with the following difference: at least one of the components of~$x$ is not copied, i.e., the copying procedure only applies to at most $n-1$ components.

			\item
				Problem~\eqref{Eq:PartialProblem} is clearly a particular case of~\eqref{Eq:GlobalProblem} and also of~\eqref{Eq:MixedProblem}.

			\item
				Follows directly from \text{(a)} and \text{(b)}.
		\end{list}
  \end{proof}
	Note that if drop the assumption that each function can take the value~$+\infty$, the classes are no longer equivalent: only the global and the mixed class are equivalent and the partial class is a particular case of both.

	\mypar{Distributed algorithms for each class}
	We now show that, in spite of the classes being all equivalent, they should be addressed separately in a distributed context. Underlying our analysis is the mechanism of how a distributed algorithm works, as explained in \cref{Ch:Introduction}. In particular, a distributed algorithm makes each node hold an estimate of the solution, which is iteratively updated after all the neighboring nodes exchange their estimates. We will therefore consider three generic distributed algorithms, one for each class, with the following designations and characteristics:
	\begin{itemize}
		\item \textit{AG} is a generic algorithm solving the global class; at each iteration, each node~$p$ broadcasts to its neighbors $n$ numbers representing its current estimate. In a similar way, it also receives~$n$ numbers from each of its neighbors.

		\item \textit{AP} is a generic algorithm solving the partial class; at each iteration, each node~$p$ broadcasts to its neighbors at most~$n_p = |S_p|$ numbers representing the estimates of the components it depends on.

		\item \textit{AM} is a generic algorithm solving the mixed class; at each iteration, each node~$p$ broadcasts to its neighbors at most~$m + q_p$ numbers, where $q_p = |S_p|$. Note that node~$p$ depends on all the components of the global part of the variable~$y \in \mathbb{R}^m$, and on~$q_p$ components of the partial part of the variable~$z \in \mathbb{R}^q$.

	\end{itemize}
  We now show that solving a problem in a given class with an algorithm designed for a different class can only  decrease communication-efficiency.
  \begin{theorem}\label{Teo:ClassificationImportance}
  \hfill

  \medskip
  \noindent
  	Let the assumptions of Lemma~\ref{lem:EquivalenceBetweenClasses} hold and consider the generic distributed algorithms AG, AP, and AM, designed for the global, partial, and mixed classes, respectively. Then,
  	\newcounter{thmClasses}
		\begin{list}{(\alph{thmClasses})}{\usecounter{thmClasses}}
			\item Solving \eqref{Eq:GlobalProblem} with AG uses less communications per iteration than solving it with AP and AM;
			\item Solving \eqref{Eq:PartialProblem} with AP uses less communications per iteration than solving it with AG and AM;
			\item Solving \eqref{Eq:MixedProblem} with AM uses less communications per iteration than solving it with AG and AP.
		\end{list}
  \end{theorem}

  \begin{proof}
  	\hfill

  	\medskip
  	\noindent
  	\newcounter{thmClassesProof}
		\begin{list}{(\alph{thmClassesProof})}{\usecounter{thmClassesProof}}
			\item
				By the definition of AG, solving \eqref{Eq:GlobalProblem} with AG makes each node broadcast~$n$ numbers to its neighbors at each iteration. In the proof of Lemma~\ref{lem:EquivalenceBetweenClasses}, we saw that recasting~\eqref{Eq:GlobalProblem} as~\eqref{Eq:PartialProblem} requires first recasting it as~\eqref{Eq:Cl:LemmaProof1}. Independently of how the equality between the copies is enforced, the resulting function~\eqref{Eq:Cl:LemmaProof3} at each node depends at least on two copies (since each node has to make its own copy equal to the copy of at least one of its neighbors). This means that the cardinality of the set~$S_p$ is at least~$2n$. As a consequence, solving~\eqref{Eq:Cl:LemmaProof2} with AP implies that each node broadcasts at least $2n$ numbers per iteration, the double of what is transmitted when \eqref{Eq:GlobalProblem} is solved with AG.

				The same reasoning can be applied to show that solving~\eqref{Eq:GlobalProblem} with AM leads to an increase of the number of communications per iteration.

			\item
				By the definition of AP, solving~\eqref{Eq:PartialProblem} with AP requires that each node broadcasts at most $n_p = |S_p|$ numbers per iteration. If AG is applied to solve~\eqref{Eq:PartialProblem}, then it makes all the nodes broadcast full solution estimates, i.e., vectors of size~$n$. Since we assume that $S_1 \cap \cdots \cap S_P = \emptyset$, then not all the sets~$S_p$ can be equal to the full set $\{1,\ldots,n\}$, which means at least one set~$S_p$ has cardinality less than $n$, i.e., $|S_p| < n$. Thus, that node will broadcast more numbers per iteration by using AG than by using AP.

				The exact same reasoning concludes that using AM to solve~\eqref{Eq:GlobalProblem} will inevitably use more communications per iteration than using AG.

			\item
			  Follows directly from \text{(a)} and \text{(b)}.
		\end{list}
  \end{proof}

  In sum, if a problem naturally fits one of the three classes, it should be solved with an algorithm that was specifically designed for that class, because reformulating problems between classes increases the size of the variable and thus the communication burden. This means that, to achieve greater efficiency, we have to address each class separately. However, this does not imply that no algorithm can be designed to solve all the classes. In fact, one of the contributions of this thesis is the design of an algorithm that solves problems in all the classes in an efficient way. The key point is that the proposed algorithm does not require reformulating problems between different classes: it just incorporates all the classes in its design.


\section{The connected and the non-connected subclasses}
\label{Sec:ConnectedAndNonConnectedSubclasses}

  \begin{figure}[h]
  \centering
  \subfigure[Connected]{\label{SubFig:ConnectedInducedSubgraph}
    \psscalebox{0.9}{
      \begin{pspicture}(4.9,4.8)
        \def\nodesimp{
          \pscircle*[linecolor=black!65!white](0,0){0.3}
        }
        \def\nodeshigh{
          \pscircle*[linecolor=black!25!white](0,0){0.3}
        }

        \rput(0.5,4.1){\rnode{C1}{\nodesimp}}    \rput(0.5,4.1){\small \textcolor{white}{$1$}}
        \rput(1.0,2.6){\rnode{C2}{\nodesimp}}    \rput(1.0,2.6){\small \textcolor{white}{$2$}}
        \rput(0.9,0.9){\rnode{C3}{\nodesimp}}    \rput(0.9,0.9){\small \textcolor{white}{$3$}}
        \rput(3.1,1.1){\rnode{C4}{\nodeshigh}}   \rput(3.1,1.1){\small \textcolor{black!60!white}{$4$}}
        \rput(4.1,2.6){\rnode{C5}{\nodeshigh}}   \rput(4.1,2.6){\small \textcolor{black!60!white}{$5$}}
        \rput(2.3,3.3){\rnode{C6}{\nodesimp}}    \rput(2.3,3.3){\small \textcolor{white}{$6$}}

        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C2}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C3}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C3}{C4}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C4}{C5}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C5}{C6}

        \rput[lb](-0.1,4.45){\small $f_1(\boldsymbol{x_1},x_2)$}
        \rput[lt](1.2,2.4){\small $f_2(\boldsymbol{x_1},x_2,x_3)$}
        \rput[lt](0,0.56){\small $f_3(\boldsymbol{x_1},x_3)$}
        \rput[t](3.1,0.74){\small \textcolor{black!70!white}{$f_4(x_3)$}}
        \rput[b](4.2,2.97){\small \textcolor{black!70!white}{$f_5(x_2,x_3)$}}
        \rput[b](2.7,3.65){\small $f_6(\boldsymbol{x_1},x_2)$}

        %\psgrid
      \end{pspicture}
    }
  }
  \hspace{2cm}
  \subfigure[Non-connected]{\label{SubFig:NonConnectedInducedSubgraph}
    \psscalebox{0.9}{
      \begin{pspicture}(4.9,4.8)
        \def\nodesimp{
          \pscircle*[linecolor=black!65!white](0,0){0.3}
        }
        \def\nodeshigh{
          \pscircle*[linecolor=black!25!white](0,0){0.3}
        }
        \rput(0.5,4.1){\rnode{C1}{\nodesimp}}   \rput(0.5,4.1){\small \textcolor{white}{$1$}}
        \rput(1.0,2.6){\rnode{C2}{\nodesimp}}   \rput(1.0,2.6){\small \textcolor{white}{$2$}}
        \rput(0.9,0.9){\rnode{C3}{\nodeshigh}}  \rput(0.9,0.9){\small \textcolor{black!60!white}{$3$}}
        \rput(3.1,1.1){\rnode{C4}{\nodesimp}}   \rput(3.1,1.1){\small \textcolor{white}{$4$}}
        \rput(4.1,2.6){\rnode{C5}{\nodeshigh}}  \rput(4.1,2.6){\small \textcolor{black!60!white}{$5$}}
        \rput(2.3,3.3){\rnode{C6}{\nodesimp}}   \rput(2.3,3.3){\small \textcolor{white}{$6$}}

        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C2}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C1}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C2}{C3}
        \ncline[nodesep=0.33cm,linewidth=0.9pt]{-}{C2}{C6}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C3}{C4}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C4}{C5}
        \ncline[nodesep=0.33cm,linewidth=0.9pt,linecolor=black!25!white]{-}{C5}{C6}

        \rput[lb](-0.1,4.45){\small $f_1(\boldsymbol{x_1},x_2)$}
        \rput[lt](1.2,2.4){\small $f_2(\boldsymbol{x_1},x_2,x_3)$}
        \rput[lt](0.2,0.56){\small \textcolor{black!70!white}{$f_3(x_2,x_3)$}}
        \rput[t](3.1,0.74){\small $f_4(\boldsymbol{x_1})$}
        \rput[b](4.2,2.97){\small \textcolor{black!70!white}{$f_5(x_2,x_3)$}}
        \rput[b](2.7,3.65){\small $f_6(\boldsymbol{x_1},x_2)$}

        %\psgrid
      \end{pspicture}
    }
  }
  \caption{
   Examples of subgraphs induced by the component $x_1$: \text{(a)} connected and \text{(b)} non-connected.
  }
  \label{Fig:SubClassesConnectedAndNonConnected}
  \end{figure}

	We saw in \fref{Fig:Classification} that the partial and the mixed classes are subdivided into two subclasses: connected and non-connected. According to the definitions of a connected and a non-connected variable, if all the components of the variable induce connected subgraphs, the variable is connected; if there is at least one component that induces a non-connected subgraph, then the variable is non-connected. Figures \ref{SubFig:ConnectedInducedSubgraph} and \ref{SubFig:NonConnectedInducedSubgraph} illustrate a connected and a non-connected induced subgraph, respectively. From these figures, it becomes clear that the connected case is easier to handle than the non-connected one, since it seems straightforward to make the nodes in the same connected subgraph exchange estimates between themselves, that is, to agree on an optimal value for the respective component.

	On the other hand, a non-connected variable requires devising a scheme to let the estimates of the non-connected components agree somehow. For example, in \fref{SubFig:NonConnectedInducedSubgraph}, even if node~$4$ broadcasts its estimate of~$x_1$ to its neighboring nodes~$3$ and~$5$, these nodes will not be interested in that estimate, since their functions do not depend on~$x_1$. So, to make the $x_1$-estimates of node~$1$ agree with the $x_1$-estimates of nodes~$1$, $2$, and~$6$, we are forced to make one of the nodes~$3$ or~$5$ receive the estimates of~$x_1$ and retransmit them to its neighbors. In the case of \fref{SubFig:NonConnectedInducedSubgraph}, it is indifferent to choose either node~$3$ or node~$5$ to perform that task. In a larger network, however, it becomes much more challenging to select these retransmission nodes such that the overall number of communications is minimized, a goal we pursue in this thesis. We will address this topic in \cref{Ch:PartialVariable} when we propose an algorithm for the partial class.











